Solving the TTC 2011 Reengineering Case with VIATRA2

The current paper presents a solution of the Program Understanding: A Reengineering Case for the Transformation Tool Contest using the VIATRA2 model transformation tool.

==> eptcsdata.tex <==
\providecommand{\firstpage}{136}
\providecommand{\publicationstatus}{Van Gorp, Mazanek and Rose (Eds.): \\Fifth Transformation Tool Contest (TTC 2011)\\
EPTCS 74, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.74.13}{10.4204/EPTCS.74.13}}
\pdfoutput=1

